Electroweak corrections to squark-antisquark production at the LHC

We present the calculation of the electroweak corrections for squark-antisquark pair production at the LHC within the Minimal Supersymmetric Standard Model. Taking into account all possible chirality and light-flavor configurations, we evaluate the NLO EW corrections, which are of O(a_s^2 a), as well as the subleading tree-level contributions of O(a_s a) and O(a^2). Numerical results are presented for several scans in the SUSY parameter space and relevant differential distributions are investigated. The impact of the electroweak corrections is nonnegligible and strongly depends on the chirality configuration of the produced squarks. Our analysis includes a discussion of photon-gluon initiated processes with a focus on the impact of the corresponding large PDF uncertainties.

==> TREES/T0u.tex <==
\unitlength=.15bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(4.78682,11.5936)[tr]{\tiny$g$}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.21318,6.59364)[tl]{\tiny$g$}
\FAProp(20.,15.)(10.,10.)(0.,){/ScalarDash}{-1}
\FALabel(14.7868,13.4064)[br]{\tiny$\tilde q_\alpha$}
\FAProp(20.,5.)(10.,10.)(0.,){/ScalarDash}{1}
\FALabel(15.2132,8.40636)[bl]{\tiny$\tilde q_\alpha$}
\FAVert(10.,10.){0}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FALabel(2.48771,11.7893)[tr]{\tiny$g$}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FALabel(3.51229,6.78926)[tl]{\tiny$g$}
\FAProp(20.,15.)(14.,10.)(0.,){/ScalarDash}{-1}
\FALabel(16.4877,13.2107)[br]{\tiny$\tilde q_\alpha$}
\FAProp(20.,5.)(14.,10.)(0.,){/ScalarDash}{1}
\FALabel(17.5123,8.21074)[bl]{\tiny$\tilde q_\alpha$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(10.,8.93)[t]{\tiny $g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\end{feynartspicture}



==> TREES/T24.tex <==
\unitlength=0.15bp%
%

%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{\tiny $q$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{\tiny $q'$}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{-1}
\FALabel(14.8458,15.5623)[b]{\tiny $\tilde q_\alpha$}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{1}
\FALabel(15.1542,6.56231)[b]{\tiny $\tilde q'_\beta$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.18,10.)[r]{\tiny $\tilde g$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}



==> TREES/TGd.tex <==
\unitlength=.15bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(4.84577,13.4377)[t]{\tiny$g$}
\FAProp(0.,5.)(10.,6.)(0.,){/Sine}{0}
\FALabel(5.15423,4.43769)[t]{\tiny$\gamma$}
\FAProp(20.,15.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(16.8128,13.2058)[br]{\tiny$\tilde q_\alpha$}
\FAProp(20.,5.)(10.,14.)(0.,){/ScalarDash}{1}
\FALabel(17.6872,8.20582)[bl]{\tiny$\tilde q_\alpha$}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{1}
\FALabel(9.03,8.8)[r]{\tiny$\tilde q_\alpha$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}
%
\color{bianco}
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(4.84577,13.4377)[t]{\tiny$g$}
\FAProp(0.,5.)(10.,6.)(0.,){/Sine}{0}
\FALabel(5.15423,4.43769)[t]{\tiny$\gamma$}
\FAProp(20.,15.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(16.8128,13.2058)[br]{\tiny$\tilde q_\alpha$}
\FAProp(20.,5.)(10.,14.)(0.,){/ScalarDash}{1}
\FALabel(17.6872,8.20582)[bl]{\tiny$\tilde q_\alpha$}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{1}
\FALabel(9.03,8.8)[r]{\tiny$\tilde q_\alpha$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}
%
\color{nero}

